Defending Against Neural Fake News

Recent progress in natural language generation has raised dual-use concerns. While applications like summarization and translation are positive, the underlying technology also might enable adversaries to generate neural fake news: targeted propaganda that closely mimics the style of real news. Modern computer security relies on careful threat modeling: identifying potential threats and vulnerabilities from an adversary's point of view, and exploring potential mitigations to these threats. Likewise, developing robust defenses against neural fake news requires us first to carefully investigate and characterize the risks of these models. We thus present a model for controllable text generation called Grover. Given a headline like `Link Found Between Vaccines and Autism,' Grover can generate the rest of the article; humans find these generations to be more trustworthy than human-written disinformation. Developing robust verification techniques against generators like Grover is critical. We find that best current discriminators can classify neural fake news from real, human-written, news with 73% accuracy, assuming access to a moderate level of training data. Counterintuitively, the best defense against Grover turns out to be Grover itself, with 92% accuracy, demonstrating the importance of public release of strong generators. We investigate these results further, showing that exposure bias -- and sampling strategies that alleviate its effects -- both leave artifacts that similar discriminators can pick up on. We conclude by discussing ethical issues regarding the technology, and plan to release Grover publicly, helping pave the way for better detection of neural fake news.

==> figures/grammyawards.tex <==
\begin{figure}[t]

Provided \domainfield: {\tt\small \href{https://latimes.com}{latimes.com}} \\
Provided \datefield: February 20, 2019 \\
Provided \headlinefield: La Jolla's Rowan Zellers wins Grammy for his first album, set to perform Sunday at The Coach House \\

\hrule
Generated \bodyfield:
{\small
Rowan Zellers won the Grammy Award for Best Alternative Album on Sunday at the Grammys. He describes it as a form of validation.

“I don’t feel that artists should be judged just off of their label’s box,” the 38-year-old La Jolla resident said from the stage, where he accepted the award in California for “Ruminations,” one of his three albums. “I truly believe that we should all be judged by our truth, and music being a reflection of who you are. So I don’t feel that ‘alternative’ is in the ‘quaint’ category. I feel that it’s so much more, and the power of the tool is so much more than anything else.”

His father, Scott, first gave him the piano when he was four years old. “He was the first person who made me feel special,” Zellers said. “He bought me a three-string guitar as well. I started playing music when I was 7. It was my adventure into the world. Music was my thing to do, and I’m so glad he gave me that gift.”
His first effort was “Summer Rose.” “It was for my grandparents. They were retired, but I was 8 years old and I went around the neighborhood and got a bunch of roses to give to my grandparents. It was completely unintentional, but I’m glad I did because I got most of them. My grandfather was 91 years old and I was playing for him. I would do it at the end of dinner, and I remember this beautiful day. It just all worked out. He knew what I was doing.”

Rowan Zellers as a boy listening to his first CD. Rowan Zellers as a boy listening to his first CD.
His father encouraged him to take piano lessons, which led to drums when he was 10. Then he took drums lessons for six months and was thoroughly inspired. “The first lesson was at a garage band in Phoenix. The whole world was around the room. The drummer was blind and he had an incredible voice.”

Ten years later, he had his first commercial recording deal and started to play shows, which led to a big record deal. “I remember playing America’s legendary Fillmore West for my first time. I was in someone else’s band and we finished our set, and there were 10,000 people standing. There was a giant crowd, and I was like, ‘Wait.’

“Then to go up on this stage with a headlining band — the Fillmore West and the Fillmore East — and my voice, my drums and all this crazy light shows from the ceiling, it was so much better than when I was in the middle of a giant group. I don’t know if I was trying to be the original drummer and it just wasn’t really working, but what it did do was that it got me more independent and it allowed me to reach further. I was only looking for a chance to be the Next Big Thing, and I was really hard on myself for not reaching it.”
Rowan Zellers performing at Coachella 2014. Rowan Zellers performing at Coachella 2014.

His work has never been commercially successful, but he doesn’t think that’s an issue. “The whole idea of selling your soul for money was really strong in my dad’s family. He grew up with a grandfather who bought me music by The Doors, The Grateful Dead and Hendrix because he knew it was his legacy. The reason why they were successful was that you didn’t actually have to sell your soul, but by that definition, not everybody wants that.

“It was very clear that my music was having a path and had a purpose, so I never, ever tried to please other people or make a commercial deal. I tried to please myself and follow my heart. I think what’s been really beautiful about having my own platform is that it allowed me to hear a lot of people like what I was doing. I feel like it’s been really cool to see the fulfillment of my vision.”
}
\caption{An example of a fake news story, generated using the first author's name, about them ostensibly winning the Grammy Award for album of the year}
\label{fig:grammyawards}
\end{figure}


==> sections/07_relatedwork.tex <==
\rowan{Maybe we can find a way to nix the RW section}

% This could go in a supp?
Related to our study are the SWAG benchmarks for natural language inference \citep{zellers2018swagaf, zellers2018hellaswag}, which involve distinguishing nonsensical, machine-written endings from human-written endings. These tasks seem significantly harder for machines than fake news discrimination (<50\% accuracy for BERT-Large in a four-way setting), likely due to HellaSwag endings being 148 BPE tokens or fewer, whereas we consider news articles within a window of 1024 tokens.

% This is already discussed earlier?
Related work has considered the task of claim verification. One popular dataset, FEVER \citep{thorne2018fever}, treats claim verification as a task where a paragraph of evidence is provided, and a sentence-long `claim' is judged true or false. An open question is to existing progress in this task towards entire news articles, where evidence is noisy (similar to open-domain QA \citealp{chen2017reading}).
